The Computational Lens: from Quantum Physics to Neuroscience

Two transformative waves of computing have redefined the way we approach science. The first wave came with the birth of the digital computer, which enabled scientists to numerically simulate their models and analyze massive datasets. This technological breakthrough led to the emergence of many sub-disciplines bearing the prefix "computational" in their names. Currently, we are in the midst of the second wave, marked by the remarkable advancements in artificial intelligence. From predicting protein structures to classifying galaxies, the scope of its applications is vast, and there can only be more awaiting us on the horizon. While these two waves influence scientific methodology at the instrumental level, in this dissertation, I will present the computational lens in science, aiming at the conceptual level. Specifically, the central thesis posits that computation serves as a convenient and mechanistic language for understanding and analyzing information processing systems, offering the advantages of composability and modularity. This dissertation begins with an illustration of the blueprint of the computational lens, supported by a review of relevant previous work. Subsequently, I will present my own works in quantum physics and neuroscience as concrete examples. In the concluding chapter, I will contemplate the potential of applying the computational lens across various scientific fields, in a way that can provide significant domain insights, and discuss potential future directions.

==> endmatter/colophon.tex <==
%!TEX root = ../dissertation.tex
\newpage

% If you do want an image in the colophon:
\begin{figure}
  \vspace{20pt}
  \centering
  \hspace*{-32pt}
  \includegraphics[width=0.42\textwidth]{endmatter/colophon.png}
\end{figure}

% If you don't want an image in the colophon:
% \vspace*{200pt}

\begin{center}
\parbox{200pt}{\lettrine[lines=3,slope=-2pt,nindent=-4pt]{\textcolor{SchoolColor}{T}}{his thesis was typeset} using \LaTeX, originally developed by Leslie Lamport and based on Donald Knuth's \TeX. The body text is set in 11 point Egenolff-Berner Garamond, a revival of Claude Garamont's humanist typeface. The above illustration, \textit{Science Experiment 02}, was created by Ben Schlitter and released under \href{http://creativecommons.org/licenses/by-nc-nd/3.0/}{\textsc{cc by-nc-nd 3.0}}. A template that can be used to format a PhD dissertation with this look \textit{\&} feel has been released under the permissive \textsc{agpl} license, and can be found online at \href{https://github.com/suchow/Dissertate}{github.com/suchow/Dissertate} or from its lead author, Jordan Suchow, at \href{mailto:suchow@post.harvard.edu}{suchow@post.harvard.edu}.}
\end{center}


==> endmatter/personalize.tex <==
%!TEX root = ../dissertation.tex


==> frontmatter/abstract.tex <==
Two transformative waves of computing have redefined the way we approach science. The first wave came with the birth of the digital computer, which enabled scientists to numerically simulate their models and analyze massive datasets. This technological breakthrough led to the emergence of many sub-disciplines bearing the prefix ``computational'' in their names. Currently, we are in the midst of the second wave, marked by the remarkable advancements in artificial intelligence. From predicting protein structures to classifying galaxies, the scope of its applications is vast, and there can only be more awaiting us on the horizon. 

While these two waves influence scientific methodology at the instrumental level, in this dissertation, I will present the computational lens in science, aiming at the conceptual level. Specifically, the central thesis posits that computation serves as a convenient and mechanistic language for understanding and analyzing information processing systems, offering the advantages of composability and modularity.

This dissertation begins with an illustration of the blueprint of the computational lens, supported by a review of relevant previous work. Subsequently, I will present my own works in quantum physics and neuroscience as concrete examples. In the concluding chapter, I will contemplate the potential of applying the computational lens across various scientific fields, in a way that can provide significant domain insights, and discuss potential future directions.


==> frontmatter/junk/dedication.tex <==
%!TEX root = ../dissertation.tex
% dedication text

%To Dilu, Mami, Tati, and Delaney. 

%And to Bianca -- the best friendships are forever.

To my parents. 

==> frontmatter/personalize.tex <==
%!TEX root = ../dissertation.tex

% Some details about the dissertation.
\title{The Computational Lens:\\ from Quantum Physics to Neuroscience}
\author{Chi-Ning Chou}
\coadvisorOne{Boaz Barak}

% ... about the degree.
\degree{Doctor of Philosophy}
\field{Computer Science}
\degreeyear{2023}
\degreemonth{June}
\department{Engineering And Applied Sciences}

% ... about the candidate's previous degrees.
\pdOneName{B.S.}
\pdOneSchool{National Taiwan University}
\pdOneYear{2016}


==> frontmatter/thanks.tex <==
One of the most profound lessons I have learned during my Ph.D. years is the fact that it is the people surround us that infuse our life's journey with vibrant hues. Therefore, I would like to take time and space here to thank all the important individuals who have played an indispensable part in my past six years.


\subsection*{Mentors}
First and foremost, I would like to express my deep gratitude to my advisor, Professor Boaz Barak. I cannot imagine having anyone else guide me through my PhD journey. You have always placed unconditional trust in me, provided me with freedom to pursue my ideas, and offered unwavering support and guidance. Even though we collaborated less on concrete research projects in the later stage of my PhD, your scientific vision and creative thinking continued to inspire me a lot. 
In particular, I am grateful for your invaluable advice, which I often initially disagreed with, but later realized its significance after a few months. Thank you, Boaz, for being a wonderful mentor and a role model for me.

Next, I would like to express my gratitude to Professor Madhu Sudan. Working with you is always enjoyable, whether it is writing papers or teaching classes. Your remarkable ability to transition seamlessly between high-level intuitions and technical details never cease to amaze me. I would also like to thank you for organizing countless spontaneous paper discussions, reading groups, and theory socials.

I would also like to thank Professor Anurag Anshu for serving on my committee. Although our time together in Harvard CS theory group was brief, spanning just over a year, I learned a great deal from you. I was especially impressed by your ability to bridge the gap between physicists and computer scientists through great communications.

I cannot forget to thank Professor Salil Vadhan, who has always been friendly and knowledgeable. I also wish to express my gratitude to the other professors with whom I have interacted from time to time and who have influenced my thinking, including Professor Cengiz Pehlevan, Professor Cynthia Dwork, Professor David Haig, Professor Jelani Nelson, Professor Lawrence Williams, and Professor Nancy Lynch.

I would like to extend my heartfelt thanks to the many senior people at Harvard theory of computation group who provided me with invaluable guidance, including Josh Alman, Jaroslaw Blasiok, Yi-Hsiu Chen, Thibaut Horel, Mrinal Kumar, Tselil Schramm, and Jiapeng Zhang.

Special thanks to Sasha Golovnev, for always patiently listening to my vague ideas and catching the bugs in my arguments. You have taught me how to be more mature in a collaboration. Although after so many years, we still haven't shown any explicit matrices to be rigid, the process has undoubtedly made our collaboration and friendship more rigid.

And I also want to specially thank Xun Gao, for teaching me so much about physics and being patient in answering all my questions. I also admire your vision and ambition in science, and I am eagerly looking forward to the future development of your research agenda.

\vspace{0.5cm}

I would also like to express my gratitude to mentors and teachers outside Harvard who have played a significant role in shaping my academic and PhD journey.

First I want to thank my former advisor Dr.~Kai-Min Chung in Taiwan for his mentorship and friendship. You are a unique researcher who always asks super insightful questions, whether he's familiar with the topic or not. From computational complexity to quantum computation and neuroscience, we always have so much to talk about, and time is never enough. Thank you for introducing me to theoretical computer science and neuroscience and encouraging me to study what I’m passionate about.

Next, I would like to thank my future postdoc supervisor, Professor SueYeon Chung, from the Flatiron Institute and NYU. I am amazed by how you can always see my strengths, which I have never realized on my own. You provide me with guidance and inputs, while also allowing me the freedom to think and figure out the big picture on my own. Your efforts to build an inclusive community are also admirable, and I am proud to be a part of it. I am very excited about the adventure that awaits us in the next few years.

I also want to express my gratitude to Professor Soonwon Choi from MIT. Your sharp thinking and broad vision always provide me with high-level scientific perspectives as well as the intuitive understandings of the details. Your enthusiasm for science and open-mindedness towards interdisciplinary research also serve as a great role model for me.

Finally, I want to thank my piano teacher Honxi Li from the Frost School of Music. In the early days of having lessons from you, I often wondered why you taught me so little and why my progress was so slow. Having been a teaching fellow for seven courses at Harvard, I thought I knew something about teaching. However, I only realized very recently how great a teacher you are. You often gave me implicit hints and guidance so that I could figure out the subtitles on my own and ``feel'' the music. Not exaggerating, your teaching has also influenced the way I think about teaching.

\subsection*{Cohorts, collaborators, and colleagues}

One aspect of academia that I particularly cherish is the camaraderie and friendship fostered among cohorts, collaborators, and colleagues.

First, I would like to thank the members from Harvard's theory of computation group for the spontaneous office discussions, theory student seminar (a.k.a., TGINF), and countless free-food hunting and extra-curricular events. I extend my special thanks to Alex Sun, Benjamin Edelman, Cassandra Marcussen, Chin Ho Lee, David Brewster, Fred Zhang, Gal Kaplun, Jake Ruotolo, Jamie Tucker-Foltz, Jaroslaw Blasiok, Jayshree Sarathy, Jenny Kaufmann, Juspreet Singh Sandhu, Kevin Rao, Mitali Bafna, Noah Singer, Pranay Tankala, Prashanth Amireddy, Prayaag Venkat, Preetum Nakkiran, Rohit Agrawal, Santhoshini Velusamy, Ted Pyne, Thibaut Horel, Yeongwoo Hwang, Yi-Hsiu Chen, Yueqi Sheng, Zachary Ratliff, and Zhixian Lei.

I would like to extend my gratitude to the former members of Kai-Min's lab in Academia Sinica: Yanlin Chen, Yu-Chi Chen, Wei-Kai Lin, and Hao Chung. During my initial years of learning theoretical computer science, your companionship and insightful discussions were transformative. Your presence and support have played a significant role in shaping me into the person I am today. I am truly grateful for the enriching experiences and the invaluable knowledge shared within our lab.

I would like to thank the members of SueYeon's lab at the Flatiron Institute: Abdulkadir Canatar, Jenelle Feather, Sonica Saraf, Nga Yu Lo, Albert Wakhloo, Yilun Kuang, and Michael Kuoch. Our collective efforts in investigating representational geometry in neuroscience have been truly inspiring. I am grateful for the collaborative atmosphere and the exciting prospects that lie ahead as we continue our journey together.

I would like to express my gratitude to the Graduate Student Council at Harvard for their support in facilitating the creation of a mini-course in January 2022. I am also immensely thankful to my friends, Lijie Chen, Xun Gao, Khadijeh Sona Najafi, Angel Hsing-Chi Hwang, Zhiqian Wang, and Brabeeba Wang, for generously giving guest lectures during the course. Additionally, I extend my appreciation to Aaron K. Clark, Aman Goel, Avantika Agarwal, Erick Galinkin, Kartikeya Arora, K Prahlad Narasimhan, Mostafa Touny, Pawan Mishra, Reijo Jaakkola, Salvador Buse, Simone Maria Giancola, and Tirukkovalluri Sri Sowmya for their invaluable contributions as teaching staff for the mini-course.

Finally, I would like to thank all my friends and collaborators from research: Alexander Golovnev, Allan Mancoo, Ameya Velingker, Amirbehshad Shahrasbi, Andres E. Lombo, Boaz Barak, Chi-Jen Lu, Christian Machens, Dan H. Sanes, Jesus E. Lares, Jiayu Zhang, Jonathan Shi, Juspreet Singh Sandhu, Kai-Min Chung, Kamalika Chaudhuri, Karl K. Berggren, Léo Varnet, Marcin Kalinowski, Matteo Castellani, Michael Kuoch, Mikhail Lukin, Mien Brabeeba Wang, Mrinal Kumar, Nancy Lynch, Nai-Hui Chia, Nihaad Paraouty, Nikhil Parthasarathy, Noam Solomon, Preetum Nakkiran, Ren Chen, Ruizhe Zhang, Sander Keemink, Santhoshini Velusamy, Soonwon Choi, SueYeon Chung, Tiancheng Yu, Tselil Schramm, Xun Gao, Yao-Yuan Yang, Yueqi Sheng, and Zhixian Lei.



\subsection*{Friends and families}
I extend my deepest gratitude to my roommate and best friend, Wei-Ping Chan, whose unwavering support and guidance have been invaluable throughout my Ph.D. journey. Your diverse skill set and dedication in research have nurtured in me a profound appreciation for biological thinking. You are also like a brother who endured my occasional immaturity while imparting valuable lessons on personal growth. I will deeply miss our late-night conversations encompassing topics such as mathematics, evolution, politics, and life itself.

I extend my sincerest gratitude to Justin Hou, whom I have known for the longest time in Boston.  You are always my scientific idol, as you are not only ambitious and hardworking in your research but also knowledgeable and open-minded in various fields. Also thank you for taking me to my first-ever lobster meal and bringing me to my first Major League Baseball game. I am immensely grateful for your humor, kindness, and unwavering friendship, and I hope you can make breakthrough on your big project very soon

I would like to thank Yao-Yuan Yang, my long-time friend from our undergraduate days in Taiwan. Despite often holding contrasting viewpoints on politics, science, and life, we have found common ground in our shared research and philosophical interests. Our conversations, spanning topics from science to food and beyond, have always been engaging and captivating.

I extend my gratitude to Juspreet Singh Sandhu. I not only learned valuable mathematical insights but also gained self-awareness through our late-night discussions over frozen yogurt. I appreciate your straightforwardness, sharpness, and enduring friendship.

I would like to thank Lijie Chen. Our conversations span a wide range of topics, from derandomization, circuit lower bounds, to logic, philosophy, cats, and life.

I would like to thank Brabeeba Mien Wang, whose boundless creativity and profound insights never cease to amaze me. Engaging in conversations about science, music, and life with you has been an enriching experience. 

I would like to thank Lisa Yang. I’m deeply impressed by your courage to making such a big jump from theoretical CS to theoretical physics. Your serious attitude to knowledge and life also has a strong impact on me. The many books that you recommended to me have helped me navigated through the challenging moments during my Ph.D.

Many thanks to all the other friends, from Cambridge, Taiwan, and other places around the world, that added color to my Ph.D. journey, including
Aishwarya Balwani, Ava Lee, Chuan-Heng Hsiao, Chun-Chen Yao, Chi-Hua Wang, Chen-Chang Liu, Eri Muramoto, Gangsim Eom, Han-Ting Yang, Hsiang Hsu, Hsuan Hsieh, Honghao Song, Hung-Tu Chen, James Yang, Jeremy Chen, Jiajia Zhao, Jin-Cheng Guu, Jingxuan Fan, Jimmy Chiu, Jimmy Hu, JiYu Zhang, Johannes Makar, Jorge Wong, Kai Wang, Kaidong Peng, Kaifeng Bu, Khadijeh Sona Najafi, Lu Zhang, Luyi Qiu, Matthew Hong, Nikhil Vyas, Po-Chen Kuo, Sabrina Drammis, Sammy Chung, Shushu Liang, Tang-Kai Lee, Teresa Huang, Terry Chen Williams, Tiancheng Yu, Ting-Ya Chang, Tushar Arora, Wei Dang, Wei-Chung Lee, Wei-Yang Chen, Wenyu Lei, Xuangui Huang, Yi Zhai, Yen-Chun Lee, Yihan Cheu, Yu-Chen Chao, Yu-Shun Hsiao, Yu-Tien Hsu, Yumeng Zhang, Zhiqian Wang, Zi Bing Pung.


Last but not least, I would like to express my heartfelt gratitude to my family for their unwavering support. Specifically, I am profoundly thankful to my parents, Hsian-Cheng and Mei-Wen, for your enduring encouragement in helping me discover my passions and allowing me to chase my dreams since my childhood. Additionally, your constant reminders to evaluate my own progress, rather than comparing it to others', have been an invaluable lesson. I want to express my heartfelt thanks to my brother, Chi-Kai. Your unwavering friendship and dedication to caring for our parents back in Taiwan has meant the world to me. Last but not least, a special thank you to my cat, Shiba. Your companionship has been an irreplaceable pillar of support throughout my PhD journey.
